An Empirical Study on Automatically Detecting AI-Generated Source Code: How Far Are We?

Artificial Intelligence (AI) techniques, especially Large Language Models (LLMs), have started gaining popularity among researchers and software developers for generating source code. However, LLMs have been shown to generate code with quality issues and also incurred copyright/licensing infringements. Therefore, detecting whether a piece of source code is written by humans or AI has become necessary. This study first presents an empirical analysis to investigate the effectiveness of the existing AI detection tools in detecting AI-generated code. The results show that they all perform poorly and lack sufficient generalizability to be practically deployed. Then, to improve the performance of AI-generated code detection, we propose a range of approaches, including fine-tuning the LLMs and machine learning-based classification with static code metrics or code embedding generated from Abstract Syntax Tree (AST). Our best model outperforms state-of-the-art AI-generated code detector (GPTSniffer) and achieves an F1 score of 82.55. We also conduct an ablation study on our best-performing model to investigate the impact of different source code features on its performance.

==> tables/llm_table_temp0.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\caption{Performance of LLM-based Approaches (Temperature = 0)}
\label{tab:llm_result_temp0}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                 & \multicolumn{4}{c|}{ChatGPT}    & \multicolumn{4}{c|}{Gemini Pro}  & \multicolumn{4}{c|}{GPT-4}      & \multicolumn{4}{c}{Mean of Every Dataset}  \\ 
\cline{2-17}
                                  & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR    & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1             \\ 
\hline
GPT-3.5 (Zero shot) - Code        & 51.73 & 99.84 & 0.00  & 33.74   & 46.16 & 100.00 & 0.00  & 31.42   & 50.43 & 98.73 & 0.00  & 33.40   & 49.44 & 99.52 & 0.00  & 32.85               \\ 
\hline
GPT-3.5 (In-context) - Code       & 51.48 & 83.23 & 20.13 & 44.56   & 40.99 & 64.91  & 20.53 & 37.66   & 53.00 & 82.58 & 22.73 & 47.14   & 48.49 & 76.91 & 21.13 & 43.12               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code       & 82.67 & 94.75 & 70.63 & 81.33   & 62.10 & 95.92  & 34.98 & 56.85   & 81.24 & 99.21 & 64.00 & 78.15   & 75.34 & 96.63 & 56.54 & 72.11               \\ 
\hline
GPT-3.5 (Zero shot) - AST         & 43.78 & 68.85 & 15.31 & 37.18   & 47.13 & 73.88  & 24.67 & 42.43   & 45.66 & 62.73 & 27.84 & 41.46   & 45.52 & 68.49 & 22.61 & 40.36               \\ 
\hline
GPT-3.5 (In-context) - AST        & 52.43 & 83.75 & 20.92 & 45.90   & 43.59 & 69.56  & 19.87 & 39.47   & 57.74 & 83.04 & 31.31 & 53.30   & 51.25 & 78.78 & 24.03 & 46.22               \\ 
\hline
GPT-3.5 (Fine-tuned) - AST        & 70.69 & 76.37 & 64.44 & 68.67   & 63.10 & 74.93  & 50.55 & 59.11   & 65.09 & 70.17 & 62.63 & 62.09   & 66.29 & 73.82 & 59.21 & 63.29               \\ 
\hline
GPT-3.5 (Zero shot) - Code + AST  & 50.98 & 96.19 & 1.25  & 34.27   & 46.23 & 98.60  & 1.70  & 32.85   & 50.58 & 97.90 & 1.43  & 34.68   & 49.26 & 97.56 & 1.46  & 33.93               \\ 
\hline
GPT-3.5 (In-context) - Code + AST & 50.93 & 53.68 & 43.60 & 46.32   & 41.80 & 55.37  & 28.99 & 38.65   & 52.65 & 66.27 & 37.73 & 49.35   & 48.46 & 58.44 & 36.77 & 44.77               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code + AST & 75.48 & 85.36 & 61.29 & 70.99   & 62.54 & 79.66  & 50.14 & 59.51   & 82.77 & 96.15 & 69.80 & 80.45   & 73.60 & 87.06 & 60.41 & 70.31               \\
\hline
\end{tabular}
}
\end{table*}

==> tables/llm_table_tempdef.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\caption{Performance of LLM-based Approaches (Default Temperature)}
\label{tab:llm_result_temp_def}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                 & \multicolumn{4}{c|}{ChatGPT}    & \multicolumn{4}{c|}{Gemini Pro} & \multicolumn{4}{c|}{GPT-4}       & \multicolumn{4}{c}{Mean of Every Dataset}  \\ 
\cline{2-17}
                                  & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1 & ACC   & TPR    & TNR   & AVG\_F1 & ACC   & TPR   & TNR   & AVG\_F1             \\ 
\hline
GPT-3.5 (Zero shot) - Code        & 52.64 & 99.90 & 2.57  & 36.60   & 51.67 & 99.81 & 0.09  & 34.10   & 54.15 & 100.00 & 0.05  & 35.11   & 52.82 & 99.90 & 0.90  & 35.27               \\ 
\hline
GPT-3.5 (In-context) - Code       & 51.71 & 81.31 & 18.50 & 44.51   & 41.19 & 66.64 & 18.01 & 37.20   & 55.58 & 83.80  & 25.76 & 49.80   & 49.49 & 77.25 & 20.76 & 43.83               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code       & 82.18 & 89.13 & 77.24 & 81.79   & 70.41 & 82.23 & 60.81 & 68.60   & 88.89 & 93.33  & 84.18 & 88.22   & 80.49 & 88.23 & 74.08 & 79.54               \\ 
\hline
GPT-3.5 (Zero shot) - AST         & 48.16 & 69.77 & 19.30 & 40.92   & 48.56 & 74.73 & 25.81 & 44.19   & 43.92 & 64.61  & 21.51 & 39.85   & 46.88 & 69.70 & 22.21 & 41.65               \\ 
\hline
GPT-3.5 (In-context) - AST        & 50.77 & 82.24 & 13.69 & 41.07   & 40.59 & 73.83 & 12.42 & 35.21   & 53.32 & 83.38  & 21.72 & 46.91   & 48.23 & 79.82 & 15.94 & 41.06               \\ 
\hline
GPT-3.5 (Fine-tuned) - AST        & 64.18 & 46.71 & 81.82 & 58.96   & 55.86 & 56.76 & 59.55 & 53.07   & 65.64 & 83.22  & 48.96 & 62.61   & 61.89 & 62.23 & 63.44 & 58.21               \\ 
\hline
GPT-3.5 (Zero shot) - Code + AST  & 55.50 & 97.78 & 4.29  & 38.78   & 44.65 & 97.54 & 0.69  & 31.30   & 52.05 & 98.19  & 1.77  & 35.51   & 50.73 & 97.84 & 2.25  & 35.20               \\ 
\hline
GPT-3.5 (In-context) - Code + AST & 46.27 & 50.71 & 40.43 & 42.90   & 37.90 & 52.01 & 22.01 & 32.70   & 52.57 & 61.81  & 43.50 & 50.25   & 45.58 & 54.84 & 35.31 & 41.95               \\ 
\hline
GPT-3.5 (Fine-tuned) - Code + AST & 75.25 & 91.68 & 57.12 & 72.57   & 63.06 & 85.23 & 44.26 & 59.37   & 75.37 & 90.42  & 61.87 & 71.72   & 71.23 & 89.11 & 54.42 & 67.89               \\
\hline
\end{tabular}
}
\end{table*}


==> tables/ml_table_temp0.tex <==
\begin{table*}
\caption{Performance of Machine Learning Classifier with Code Metrics (Temperature = 0)}
\label{tab:ml_result_temp0}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}           & \multicolumn{6}{c|}{ChatGPT}                    & \multicolumn{6}{c}{Gemini Pro}                  \\ 
\cline{2-13}
                            & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (RandomForestClassifier) & 82.07 & 83.95 & 78.75 & 82.41 & 79.04 & 80.73   & 66.84 & 72.72 & 64.93 & 65.15 & 67.29 & 66.22    \\ 
\hline
\multirow{2}{*}{}           & \multicolumn{6}{c|}{GPT-4}                      & \multicolumn{6}{c}{Mean of Every Dataset}       \\ 
\cline{2-13}
                            & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (RandomForestClassifier) & 71.33 & 69.25 & 74.58 & 69.41 & 71.46 & 70.44   & 73.41 & 75.31 & 72.75 & 72.33 & 72.60 & 72.46    \\
\hline
\end{tabular}
}
\end{table*}

==> tables/ml_table_tempdef.tex <==
\begin{table*}
\caption{Performance of Machine Learning Classifier with Code Metrics (Default Temperature)}
\label{tab:ml_result_tempdef}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}               & \multicolumn{6}{c|}{ChatGPT}                    & \multicolumn{6}{c}{Gemini Pro}                  \\ 
\cline{2-13}
                                & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (GradientBoostingClassifier) & 78.72 & 84.81 & 73.62 & 80.43 & 76.14 & 78.28   & 72.78 & 81.10 & 65.89 & 72.69 & 72.14 & 72.41    \\ 
\hline
\multirow{2}{*}{}               & \multicolumn{6}{c|}{GPT-4}                      & \multicolumn{6}{c}{Mean of Averages}            \\ 
\cline{2-13}
                                & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1 & ACC   & TPR   & TNR   & H\_F1 & A\_F1 & AVG\_F1  \\ 
\hline
ML (GradientBoostingClassifier) & 76.03 & 78.82 & 72.52 & 76.04 & 75.09 & 75.57   & 75.84 & 81.58 & 70.68 & 76.38 & 74.46 & 75.42    \\
\hline
\end{tabular}
}
\end{table*}

==> tables/overall_table_temp0.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}


\begin{table*}
\centering
\caption{Overall Performance Comparison (Temperature = 0)}
\label{tab:overall_result_temp0}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l} 
\hline
\multirow{2}{*}{}                              & \multicolumn{4}{c|}{\textbf{ChatGPT}}                               & \multicolumn{4}{c|}{\textbf{Gemini Pro}}                            & \multicolumn{4}{c|}{\textbf{GPT-4}}                                 & \multicolumn{4}{c}{\textbf{Overall Average}}                         \\ 
\cline{2-17}
                                               & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1} & \textbf{ACC}   & \textbf{TPR}   & \textbf{TNR}   & \textbf{AVG\_F1}  \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - Code}           & 82.67          & \textbf{94.75} & 70.63          & 81.33            & 62.10          & \textbf{95.92} & 34.98          & 56.85            & 81.24          & \textbf{99.21} & 64.00          & 78.15            & 75.34          & \textbf{96.63} & 56.54          & 72.11             \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - AST}            & 70.69          & 76.37          & 64.44          & 68.67            & 63.10          & 74.93          & 50.55          & 59.11            & 65.09          & 70.17          & 62.63          & 62.09            & 66.29          & 73.82          & 59.21          & 63.29             \\ 
\hline
\textbf{ChatGPT (Fine-tuned) - Code + AST}     & 75.48          & 85.36          & 61.29          & 70.99            & 62.54          & 79.66          & 50.14          & 59.51            & 82.77          & 96.15          & 69.80          & 80.45            & 73.60          & 87.06          & 60.41          & 70.31             \\ 
\hline
\textbf{Code Metrics (RandomForestClassifier)} & 82.07          & 83.95          & 78.75          & 80.73            & 66.84          & 72.72          & 64.93          & 66.22            & 71.33          & 69.25          & 74.58          & 70.44            & 73.41          & 75.31          & 72.75          & 72.46             \\ 
\hline
\textbf{Code Embedding - Code}                 & 87.49          & 89.69          & \textbf{85.27} & 86.61            & 68.67          & 56.76          & \textbf{75.27} & 63.32            & 82.37          & 90.87          & 75.53          & 79.94            & 79.51          & 79.11          & \textbf{78.69} & 76.62             \\ 
\hline
\textbf{Code Embedding - AST}                  & \textbf{88.79} & 93.96          & 80.93          & \textbf{87.44}   & \textbf{72.63} & 82.73          & 64.56          & \textbf{72.25}   & 81.85          & 85.67          & 78.17          & 81.80            & \textbf{81.09} & 87.45          & 74.55          & \textbf{80.50}    \\ 
\hline
\textbf{Code Embedding - Code + AST}           & 86.65          & 88.16          & 82.93          & 85.34            & 63.10          & 66.95          & 60.14          & 62.91            & \textbf{84.48} & 85.56          & \textbf{83.71} & \textbf{84.41}   & 78.07          & 80.22          & 75.59          & 77.55             \\
\hline
\end{tabular}
}
\end{table*}

==> todo.tex <==
TODO:

- Make rows blue -> DONE
- Add explanation for not conducting 2-3, 2-4 since the performance is different and generated from different models. Distance with human -> DONE
- Statistical analysis for Table VIII -> DONE
- Report size of code for Within vs Across (LOC, size of AST) -> DONE
- Write a paragraph in Discussion - for across experiment (This result is expected as this is observed in defect prediction ..) -> DONE

- Write new analysis in METHOD -> DONE
- Split paragraph from "The results ..." in Results.D -> DONE
- Add citations -> DONE
- Check Response letter
